Multilevel Modelling and Domain-Specific Languages

Modern software engineering deals with demanding problems that yield large and complex software. The area of Model-Driven Software Engineering tackles this issue by using models during the development process, but it does not address some of the communication problems among different stakeholders. Domain-Specific Modelling Languages (DSML) aim at involving domain experts with non-technical profiles in that process. DSMLs define concepts with different levels of abstraction, but traditional modelling does not allow enough flexibility to organise them adequately. Multilevel Modelling (MLM) approaches provide an unbounded number of levels of abstraction, plus other features that perfectly fit DSMLs. Their development can also benefit from Model Transformations (MT), especially when these encode the behaviour of DSMLs. MTs can be exploited by MLM, becoming a precise and reusable definition of behaviour. This thesis presents a MLM and Multilevel MT approach which tackles open issues in the field and compares it with the state of the art through literature review and experiments, providing its formalisation and its implementation in the tool MultEcore, together with case studies.

==> styles/framework-styles.tex <==
\usetikzlibrary{arrows,arrows.meta,backgrounds,positioning,calc,intersections,shapes}


\def\h{7ex}
\def\w{8em}
\def\sep{60mm}


\colorlet{editor-grey}{black!30}
\colorlet{window-grey-draw}{black!30}
\colorlet{window-grey-fill}{black!10}


\tikzset{model/.style={draw,fill=white,inner sep=4pt,minimum height=\h,minimum width=\w}}
\tikzset{model2/.style={model,rectangle split,rectangle split parts=2, rectangle split draw splits=false}}
\tikzset{editor/.style={fill=editor-grey,rounded corners,draw,inner sep=2pt,minimum height=\h,minimum width=\w}}
\tikzset{window/.style={draw=window-grey-draw,fill=window-grey-fill,fill opacity=0.5}}

\tikzset{arrow/.style={->,>=latex',semithick}}
\tikzset{conf/.style={arrow,dashed}}
\tikzset{creates/.style={arrow}}
\tikzset{typed/.style={arrow,dotted}}
\tikzset{meftrans/.style={arrow,loosely dashed, <->}}

\tikzset{label/.style={auto,midway,font=\it}}
\tikzset{label2/.style={label,midway,below}}
\tikzset{label3/.style={midway,font=\it,below,inner sep=2pt}}


% #1 = node to split
\newcommand{\splitnode}[1]{
	\draw[dotted] (#1.text split west) -- (#1.text split east);
}


==> styles/multecore-styles.tex <==
\usetikzlibrary{arrows,positioning,backgrounds,shapes,decorations.markings,calc,intersections}

\definecolor{node-yellow}{RGB}{255,245,181}
\definecolor{type-blue}{RGB}{194,239,255}
\definecolor{type-green}{RGB}{204,242,166}
\definecolor{potency-red}{RGB}{246,139,139}

\tikzset{separator/.style={thick}}
\tikzset{block-separator/.style={separator}}
\tikzset{level-separator/.style={separator,red}}
\tikzset{level/.style={font=\sffamily}}
\tikzset{model/.style={font=\sffamily\bfseries,inner sep=4pt}}
\tikzset{me-node/.style={fill=node-yellow,inner sep=2pt,minimum height=1.4em,minimum width=4em,font=\ttfamily}}
\tikzset{me-type/.style={shape=ellipse,fill=type-blue,inner sep=0pt,minimum width=2em,font=\ttfamily\tiny}}
\tikzset{me-a-type/.style={me-type,fill=type-blue}}
\tikzset{me-s-type/.style={me-type,fill=type-green}}
\tikzset{me-d-type/.style={me-type,fill=white,draw}}
\tikzset{me-potency/.style={fill=potency-red,inner sep=0pt,minimum height=1.1ex,font=\ttfamily\tiny}}
\tikzset{rel/.style={semithick}}
\tikzset{me-rel/.style={rel,->,>=latex'}}
\tikzset{me-inh/.style={rel,->,>=open triangle 60}}
\tikzset{label/.style={auto,midway,font=\ttfamily}}
\tikzset{label2/.style={auto,midway,font=\ttfamily\itshape}}
\tikzset{labelp/.style={white,background default text=white,background text=black}}

% #1 = node to add type ellipse to; #2 = type
\providecommand{\metype}[2]{
	\node[me-a-type] (type) [right=0mm of #1.north west] {#2};
}
\providecommand{\mestype}[2]{
	\node[me-s-type] (type) [right=0mm of #1.north west] {#2};
}
\providecommand{\medtype}[2]{
	\node[me-d-type] (type) [right=0mm of #1.north west] {#2};
}

% #1 = node to add potency rectangle to; #2 = potency start; #3 = potency end; #4 = potency depth
\providecommand{\mepotency}[4]{
	\node[me-potency] (type) [left=0mm of #1.north east] {#2-#3-#4};
}



==> styles/robolang-mcmts-styles.tex <==
\usetikzlibrary{arrows,backgrounds,positioning,calc,intersections,shapes}

\tikzset{box/.style={inner sep=1pt, minimum height=1.2em}}
\tikzset{node/.style={box, minimum width=9ex, semithick, rectangle}}
\tikzset{split/.style={rectangle split, rectangle split parts=2, rectangle split draw splits=true}}
\tikzset{split2/.style={rectangle split, rectangle split horizontal, rectangle split parts=2, rectangle split draw splits=true}}
\tikzset{arrow/.style={->, >=latex', semithick}}
\tikzset{label/.style={auto,midway,above}}

\tikzset{system/.style={}}
\tikzset{system-split/.style={system, split}}
\tikzset{agent/.style={thick}}
\tikzset{task/.style={node, fill=black!10, draw}}
\tikzset{initial/.style={inner sep=0pt, minimum size=3mm, circle, fill=black, draw}}
\tikzset{input/.style={node, fill=red!10, draw=red, text=red}}
\tikzset{message/.style={fill=blue!10, draw=blue, text=blue}}
\tikzset{messageguard/.style={box, blue}}
\tikzset{timedguard/.style={box, draw=blue, text=blue}}
\tikzset{timedguard-split/.style={timedguard, split, draw=blue, text=blue}}

\tikzset{transition/.style={arrow}}
\tikzset{message-1/.style={semithick, dashed, blue}}
\tikzset{message-2/.style={arrow, dashed, blue}}
\tikzset{input-1/.style={semithick, dashed, red}}
\tikzset{timed-1/.style={semithick, dashed, blue}}

\tikzset{label/.style={auto,midway,above}}
\tikzset{label-input/.style={label,text=red}}
\tikzset{label-message/.style={label,text=blue}}


% #1 = top-left limit; #2 = bottom-right limit; #3 = label text; #4 = id prefix
\providecommand{\agent}[5][]{
	\coordinate[above left=8mm and 3mm of #2] (#5-topleft);
	\coordinate[below right=4mm and 3mm of #3] (#5-bottomright);
	\path (#5-topleft) -| (#5-bottomright) coordinate[midway] (#5-topright);
	\path (#5-topleft) |- (#5-bottomright) coordinate[midway] (#5-bottomleft);
	\path (#5-topleft) -- (#5-topright) coordinate[midway] (#5-midtop);
	\path (#5-bottomleft) -- (#5-bottomright) coordinate[midway] (#5-midbottom);
	\path (#5-topleft) -- (#5-bottomleft) coordinate[midway] (#5-midleft);
	\path (#5-topright) -- (#5-bottomright) coordinate[midway] (#5-midright);
	\path (#5-topleft) -- (#5-bottomright) coordinate[midway] (#5-center);
	\draw[agent] (#5-topleft) rectangle (#5-bottomright);
	\node (#5-label) [below right=0 of #5-topleft, anchor=north west] {#4};
	\ifstrempty{#1}{}{
		\draw[color=blue,fill=blue] (#5-topleft -| #5-bottomright) ++(-1mm,-1mm) --  + (-2mm,0) -- ++ (0,-2mm) -- cycle;
	}
}


% #1 = left point of the horizontal line;
% #2 = right point of the horizontal line (only X component taken into consideration);
% #3 = bottom point of the vertical line
\providecommand{\separators}[3]{%
	\draw[thick]	(#1) -- ++(8mm,0) node[auto,above]{META} node[auto,below]{FROM} -- (#1 -| #3) -- ++(5mm,0) node[auto,below]{TO}-- (#1 -| #2);
	\draw[thick]	(#1 -| #3) -- (#3);
}


% #1 = a node of style "system-split"
\providecommand{\systemseparator}[1]{
	\draw[black] (#1.text split west) -- (#1.text split east);
}

